Multimodal Contextualized Plan Prediction for Embodied Task Completion

Task planning is an important component of traditional robotics systems enabling robots to compose fine grained skills to perform more complex tasks. Recent work building systems for translating natural language to executable actions for task completion in simulated embodied agents is focused on directly predicting low level action sequences that would be expected to be directly executable by a physical robot. In this work, we instead focus on predicting a higher level plan representation for one such embodied task completion dataset - TEACh, under the assumption that techniques for high-level plan prediction from natural language are expected to be more transferable to physical robot systems. We demonstrate that better plans can be predicted using multimodal context, and that plan prediction and plan execution modules are likely dependent on each other and hence it may not be ideal to fully decouple them. Further, we benchmark execution of oracle plans to quantify the scope for improvement in plan prediction models.

==> tables/old_results_table.tex <==
\begin{table*}[!h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
  \textbf{Models} &
  \textbf{Split} &
  \textbf{SR} &
  \textbf{GC} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Edit \\ Distance\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Pred-Length \\ Normalized \\ Edit Distance \\ (P-LNed)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}GT-Length \\ Normalized \\ Edit Distance \\ (GT-LNed)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Invalid \\ Interaction\\ Probability\end{tabular}} \\ \midrule
\multirow{2}{*}{ET (EDH baseline)} &
  Valid Seen &
  0.079 &
  0.072 &
  - &
  - &
  - &
   \\
 &
  Valid Unseen &
  0.062 &
  0.042 &
  - &
  - &
  - &
   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BART Language \\ Only\end{tabular}} &
  Valid Seen &
   &
   &
  13.807 &
   &
   &
   \\
 &
  Valid Unseen &
   &
   &
  13.992 &
   &
   &
   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ET Teacher \\ Forcing\end{tabular}} &
  Valid Seen &
  0.192 &
  0.239 &
  3.836 &
  1.022 &
  0.798 &
  0.10 \\
 &
  Valid Unseen &
  - &
  - &
  3.881 &
  0.99 &
  0.781 &
  0.11 \\ \midrule
\multirow{2}{*}{ET Obj Nav} &
  Valid Seen &
  0.132 &
  0.142 &
  32.382 &
  0.933 &
  14.624 &
  0.1175 \\
 &
  Valid Unseen &
  0.119 &
  0.130 &
  34.526 &
  0.93 &
  15.749 &
  0.09 \\ \midrule
\multirow{2}{*}{ET Obj Nav + Hier} &
  Valid Seen &
  0.127 &
  0.138 &
  34.345 &
  0.934 &
  15.535 &
  0.1098 \\
 &
  Valid Unseen &
  0.123 &
  0.149 &
  34.998 &
  0.925 &
  16.001 &
  0.1094 \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ET Obj Nav + \\ Invalid Action Mask\end{tabular}} &
  Valid Seen &
  0.137 &
  0.155 &
  35.676 &
  0.936 &
  15.816 &
  0.0000 \\
 &
  Valid Unseen &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Assist + ET\\ Teacher-Forcing\end{tabular}} &
  Valid Seen &
  0.416 &
  0.551 &
  1.38 &
   &
   &
   \\
 &
  Valid Unseen &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Assist + \\ ET Obj Nav\end{tabular}} &
  Valid Seen &
  0.150 &
  0.231 &
  52.242 &
  0.946 &
  24.311 &
  0.1102 \\
 &
  Valid Unseen &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Assist + ET Obj Nav + \\ Hier\end{tabular}} &
  Valid Seen &
  0.163 &
  0.215 &
  52.582 &
  0.951 &
  24.186 &
  0.1146 \\
 &
  Valid Unseen &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Assist + ET Obj Nav + \\ Invalid Action Mask\end{tabular}} &
  Valid Seen &
  0.161 &
  0.295 &
  58.592 &
  0.944 &
  26.948 &
  0.0000 \\
 &
  Valid Unseen &
   &
   &
   &
   &
   &
  \multicolumn{1}{l}{} \\ \bottomrule 
\end{tabular}%
}
\caption{This table shows the results of the experiments.}
\label{tab:results}
\end{table*}

==> todo.tex <==
Done -check the hierarchical model description, we want to make it more clear that we expect why this would produce more valid actions

-Done - table remove the frac GT prefix

Done -put the appendix for normalized distance to the main paper.

-Done - copy the modified table 5 into table 2 but remove SR and GC cols to avoid repetition

Done - cite the papers mentioned in the reviews
The paper should cite "From Skills to Symbols" (https://cs.brown.edu/people/gdk/pubs/orig_sym_jair.pdf), this work learns state representations to evaluate action success and validity in task planning. This paper (https://nakulgopalan.github.io/docs/language_to_symbols_camera_ready.pdf) that learns navigation skills and map natural language to them should also be cited.

-qualitative comparison between the baseline and E.T. models.
